PDPP: Projected Diffusion for Procedure Planning in Instructional Videos

In this paper, we study the problem of procedure planning in instructional videos, which aims to make a plan (i.e. a sequence of actions) given the current visual observation and the desired goal. Previous works cast this as a sequence modeling problem and leverage either intermediate visual observations or language instructions as supervision to make autoregressive planning, resulting in complex learning schemes and expensive annotation costs. To avoid intermediate supervision annotation and error accumulation caused by planning autoregressively, we propose a diffusion-based framework, coined as PDPP, to directly model the whole action sequence distribution with task label as supervision instead. Our core idea is to treat procedure planning as a distribution fitting problem under the given observations, thus transform the planning problem to a sampling process from this distribution during inference. The diffusion-based modeling approach also effectively addresses the uncertainty issue in procedure planning. Based on PDPP, we further apply joint training to our framework to generate plans with varying horizon lengths using a single model and reduce the number of training parameters required. We instantiate our PDPP with three popular diffusion models and investigate a series of condition-introducing methods in our framework, including condition embeddings, MoEs, two-stage prediction and Classifier-Free Guidance strategy. Finally, we apply our PDPP to the Visual Planners for human Assistance problem which requires the goal specified in natural language rather than visual observation. We conduct experiments on challenging datasets of different scales and our PDPP model achieves the state-of-the-art performance on multiple metrics, even compared with those strongly-supervised counterparts. These results further demonstrates the effectiveness and generalization ability of our model.

==> ref.tex <==
\bibitem{DBLP:conf/eccv/ChangHXAFN20}
C.~Chang, D.~Huang, D.~Xu, E.~Adeli, L.~Fei{-}Fei, and J.~C. Niebles,
  ``Procedure planning in instructional videos,'' in \emph{{ECCV} {(11)}}, ser.
  Lecture Notes in Computer Science, vol. 12356.\hskip 1em plus 0.5em minus
  0.4em\relax Springer, 2020, pp. 334--350.

\bibitem{patel2023pretrained}
D.~Patel, H.~Eghbalzadeh, N.~Kamra, M.~L. Iuzzolino, U.~Jain, and R.~Desai,
  ``Pretrained language models as visual planners for human assistance,''
  \emph{arXiv preprint arXiv:2304.09179}, 2023.

\bibitem{DBLP:conf/iccv/BiLX21}
J.~Bi, J.~Luo, and C.~Xu, ``Procedure planning in instructional videos via
  contextual modeling and model-based policy learning,'' in
  \emph{{ICCV}}.\hskip 1em plus 0.5em minus 0.4em\relax {IEEE}, 2021, pp.
  15\,591--15\,600.

\bibitem{DBLP:journals/corr/BaKH16}
L.~J. Ba, J.~R. Kiros, and G.~E. Hinton, ``Layer normalization,'' \emph{CoRR},
  vol. abs/1607.06450, 2016.


\bibitem{DBLP:conf/nips/HoJA20}
J.~Ho, A.~Jain, and P.~Abbeel, ``Denoising diffusion probabilistic models,'' in
  \emph{NeurIPS}, 2020.

\bibitem{DBLP:conf/icml/NicholD21}
A.~Q. Nichol and P.~Dhariwal, ``Improved denoising diffusion probabilistic
  models,'' in \emph{{ICML}}, ser. Proceedings of Machine Learning Research,
  vol. 139.\hskip 1em plus 0.5em minus 0.4em\relax {PMLR}, 2021, pp.
  8162--8171.

\bibitem{wang2023pdppprojected}
H.~Wang, Y.~Wu, S.~Guo, and L.~Wang, ``Pdpp:projected diffusion for procedure
  planning in instructional videos,'' in \emph{{CVPR}}, 2023.

\bibitem{DBLP:conf/nips/DhariwalN21}
P.~Dhariwal and A.~Q. Nichol, ``Diffusion models beat gans on image
  synthesis,'' in \emph{NeurIPS}, 2021, pp. 8780--8794.

\bibitem{DBLP:journals/corr/abs-2207-12598}
J.~Ho and T.~Salimans, ``Classifier-free diffusion guidance,'' \emph{CoRR},
  vol. abs/2207.12598, 2022.

\bibitem{DBLP:conf/icml/JannerDTL22}
M.~Janner, Y.~Du, J.~B. Tenenbaum, and S.~Levine, ``Planning with diffusion for
  flexible behavior synthesis,'' in \emph{{ICML}}, ser. Proceedings of Machine
  Learning Research, vol. 162.\hskip 1em plus 0.5em minus 0.4em\relax {PMLR},
  2022, pp. 9902--9915.

\bibitem{rombach2021highresolution}
R.~Rombach, A.~Blattmann, D.~Lorenz, P.~Esser, and B.~Ommer, ``High-resolution
  image synthesis with latent diffusion models,'' 2021.

\bibitem{DBLP:journals/corr/abs-2305-13311}
H.~Lu, G.~Yang, N.~Fei, Y.~Huo, Z.~Lu, P.~Luo, and M.~Ding, ``{VDT:} an
  empirical study on video diffusion with transformers,'' \emph{CoRR}, vol.
  abs/2305.13311, 2023.

\bibitem{DBLP:conf/miccai/RonnebergerFB15}
O.~Ronneberger, P.~Fischer, and T.~Brox, ``U-net: Convolutional networks for
  biomedical image segmentation,'' in \emph{{MICCAI} {(3)}}, ser. Lecture Notes
  in Computer Science, vol. 9351.\hskip 1em plus 0.5em minus 0.4em\relax
  Springer, 2015, pp. 234--241.

\bibitem{DBLP:conf/cvpr/LiangWZY22}
C.~Liang, W.~Wang, T.~Zhou, and Y.~Yang, ``Visual abductive reasoning,'' in
  \emph{{CVPR}}.\hskip 1em plus 0.5em minus 0.4em\relax {IEEE}, 2022, pp.
  15\,544--15\,554.

\bibitem{DBLP:conf/cvpr/LohRF22}
S.~B. Loh, D.~Roy, and B.~Fernando, ``Long-term action forecasting using
  multi-headed attention-based variational recurrent neural networks,'' in
  \emph{{CVPR} Workshops}.\hskip 1em plus 0.5em minus 0.4em\relax {IEEE}, 2022,
  pp. 2418--2426.

\bibitem{DBLP:conf/dagm/FarhaKSG20}
Y.~A. Farha, Q.~Ke, B.~Schiele, and J.~Gall, ``Long-term anticipation of
  activities with cycle consistency,'' in \emph{{GCPR}}, ser. Lecture Notes in
  Computer Science, vol. 12544.\hskip 1em plus 0.5em minus 0.4em\relax
  Springer, 2020, pp. 159--173.

\bibitem{DBLP:conf/nips/ZhuZWWLWD22}
J.~Zhu, X.~Zhu, W.~Wang, X.~Wang, H.~Li, X.~Wang, and J.~Dai,
  ``Uni-perceiver-moe: Learning sparse generalist models with conditional
  moes,'' in \emph{NeurIPS}, 2022.

\bibitem{DBLP:conf/wacv/MascaroAL23}
E.~V. Mascaro, H.~Ahn, and D.~Lee, ``Intention-conditioned long-term human
  egocentric action anticipation,'' in \emph{{WACV}}.\hskip 1em plus 0.5em
  minus 0.4em\relax {IEEE}, 2023, pp. 6037--6046.

\bibitem{DBLP:journals/tip/ZhaoRTZL22}
W.~Zhao, Y.~Rao, Y.~Tang, J.~Zhou, and J.~Lu, ``Videoabc: {A} real-world video
  dataset for abductive visual reasoning,'' \emph{{IEEE} Trans. Image
  Process.}, vol.~31, pp. 6048--6061, 2022.

\bibitem{DBLP:conf/iclr/ShazeerMMDLHD17}
N.~Shazeer, A.~Mirhoseini, K.~Maziarz, A.~Davis, Q.~V. Le, G.~E. Hinton, and
  J.~Dean, ``Outrageously large neural networks: The sparsely-gated
  mixture-of-experts layer,'' in \emph{{ICLR} (Poster)}.\hskip 1em plus 0.5em
  minus 0.4em\relax OpenReview.net, 2017.

\bibitem{DBLP:journals/tip/AbbasA20}
A.~Abbas and Y.~Andreopoulos, ``Biased mixtures of experts: Enabling computer
  vision inference under data transfer limitations,'' \emph{{IEEE} Trans. Image
  Process.}, vol.~29, pp. 7656--7667, 2020.

\bibitem{DBLP:conf/nips/YangBLN19}
B.~Yang, G.~Bender, Q.~V. Le, and J.~Ngiam, ``Condconv: Conditionally
  parameterized convolutions for efficient inference,'' in \emph{NeurIPS},
  2019, pp. 1305--1316.

\bibitem{DBLP:conf/nips/RiquelmePMNJPKH21}
C.~Riquelme, J.~Puigcerver, B.~Mustafa, M.~Neumann, R.~Jenatton, A.~S. Pinto,
  D.~Keysers, and N.~Houlsby, ``Scaling vision with sparse mixture of
  experts,'' in \emph{NeurIPS}, 2021, pp. 8583--8595.

\bibitem{DBLP:conf/nips/ShazeerCPTVKHLH18}
N.~Shazeer, Y.~Cheng, N.~Parmar, D.~Tran, A.~Vaswani, P.~Koanantakool,
  P.~Hawkins, H.~Lee, M.~Hong, C.~Young, R.~Sepassi, and B.~A. Hechtman,
  ``Mesh-tensorflow: Deep learning for supercomputers,'' in \emph{NeurIPS},
  2018, pp. 10\,435--10\,444.

\bibitem{DBLP:conf/iclr/LepikhinLXCFHKS21}
D.~Lepikhin, H.~Lee, Y.~Xu, D.~Chen, O.~Firat, Y.~Huang, M.~Krikun, N.~Shazeer,
  and Z.~Chen, ``Gshard: Scaling giant models with conditional computation and
  automatic sharding,'' in \emph{{ICLR}}.\hskip 1em plus 0.5em minus
  0.4em\relax OpenReview.net, 2021.

\bibitem{DBLP:conf/icra/FinnL17}
C.~Finn and S.~Levine, ``Deep visual foresight for planning robot motion,'' in
  \emph{{ICRA}}.\hskip 1em plus 0.5em minus 0.4em\relax {IEEE}, 2017, pp.
  2786--2793.

\bibitem{DBLP:conf/icml/SrinivasJALF18}
A.~Srinivas, A.~Jabri, P.~Abbeel, S.~Levine, and C.~Finn, ``Universal planning
  networks: Learning generalizable representations for visuomotor control,'' in
  \emph{{ICML}}, ser. Proceedings of Machine Learning Research, vol.~80.\hskip
  1em plus 0.5em minus 0.4em\relax {PMLR}, 2018, pp. 4739--4748.

\bibitem{DBLP:journals/ral/SunHLLZG22}
J.~Sun, D.~Huang, B.~Lu, Y.~Liu, B.~Zhou, and A.~Garg, ``Plate:
  Visually-grounded planning with transformers in procedural tasks,''
  \emph{{IEEE} Robotics Autom. Lett.}, vol.~7, no.~2, pp. 4924--4930, 2022.

\bibitem{DBLP:conf/cvpr/0004HDDWJ22}
H.~Zhao, I.~Hadji, N.~Dvornik, K.~G. Derpanis, R.~P. Wildes, and A.~D. Jepson,
  ``P\({}^{\mbox{3}}\)iv: Probabilistic procedure planning from instructional
  videos with weak supervision,'' in \emph{{CVPR}}.\hskip 1em plus 0.5em minus
  0.4em\relax {IEEE}, 2022, pp. 2928--2938.

\bibitem{DBLP:conf/nips/VaswaniSPUJGKP17}
A.~Vaswani, N.~Shazeer, N.~Parmar, J.~Uszkoreit, L.~Jones, A.~N. Gomez,
  L.~Kaiser, and I.~Polosukhin, ``Attention is all you need,'' in
  \emph{{NIPS}}, 2017, pp. 5998--6008.

\bibitem{DBLP:conf/nips/GoodfellowPMXWOCB14}
I.~J. Goodfellow, J.~Pouget{-}Abadie, M.~Mirza, B.~Xu, D.~Warde{-}Farley,
  S.~Ozair, A.~C. Courville, and Y.~Bengio, ``Generative adversarial nets,'' in
  \emph{{NIPS}}, 2014, pp. 2672--2680.

\bibitem{DBLP:conf/icml/Sohl-DicksteinW15}
J.~Sohl{-}Dickstein, E.~A. Weiss, N.~Maheswaranathan, and S.~Ganguli, ``Deep
  unsupervised learning using nonequilibrium thermodynamics,'' in
  \emph{{ICML}}, ser. {JMLR} Workshop and Conference Proceedings,
  vol.~37.\hskip 1em plus 0.5em minus 0.4em\relax JMLR.org, 2015, pp.
  2256--2265.

\bibitem{radford2019language}
A.~Radford, J.~Wu, R.~Child, D.~Luan, D.~Amodei, and I.~Sutskever, ``Language
  models are unsupervised multitask learners,'' 2019.

\bibitem{DBLP:journals/corr/abs-2204-03458}
J.~Ho, T.~Salimans, A.~A. Gritsenko, W.~Chan, M.~Norouzi, and D.~J. Fleet,
  ``Video diffusion models,'' \emph{CoRR}, vol. abs/2204.03458, 2022.

\bibitem{DBLP:journals/corr/abs-2210-02303}
J.~Ho, W.~Chan, C.~Saharia, J.~Whang, R.~Gao, A.~A. Gritsenko, D.~P. Kingma,
  B.~Poole, M.~Norouzi, D.~J. Fleet, and T.~Salimans, ``Imagen video: High
  definition video generation with diffusion models,'' \emph{CoRR}, vol.
  abs/2210.02303, 2022.

\bibitem{DBLP:journals/corr/abs-2107-00630}
D.~P. Kingma, T.~Salimans, B.~Poole, and J.~Ho, ``Variational diffusion
  models,'' \emph{CoRR}, vol. abs/2107.00630, 2021.

\bibitem{DBLP:journals/corr/abs-2209-14916}
G.~Tevet, S.~Raab, B.~Gordon, Y.~Shafir, D.~Cohen{-}Or, and A.~H. Bermano,
  ``Human motion diffusion model,'' \emph{CoRR}, vol. abs/2209.14916, 2022.

\bibitem{DBLP:journals/corr/abs-2207-09983}
D.~Yang, J.~Yu, H.~Wang, W.~Wang, C.~Weng, Y.~Zou, and D.~Yu, ``Diffsound:
  Discrete diffusion model for text-to-sound generation,'' \emph{CoRR}, vol.
  abs/2207.09983, 2022.

\bibitem{DBLP:journals/corr/ChenW15a}
Y.~Chen and M.~J. Wainwright, ``Fast low-rank estimation by projected gradient
  descent: General statistical and algorithmic guarantees,'' \emph{CoRR}, vol.
  abs/1509.03025, 2015.

\bibitem{DBLP:conf/allerton/HauswirthBHD16}
A.~Hauswirth, S.~Bolognani, G.~Hug, and F.~D{\"{o}}rfler, ``Projected gradient
  descent on riemannian manifolds with applications to online power system
  optimization,'' in \emph{Allerton}.\hskip 1em plus 0.5em minus 0.4em\relax
  {IEEE}, 2016, pp. 225--232.

\bibitem{DBLP:conf/icip/DengK20}
Y.~Deng and L.~J. Karam, ``Universal adversarial attack via enhanced projected
  gradient descent,'' in \emph{{ICIP}}.\hskip 1em plus 0.5em minus 0.4em\relax
  {IEEE}, 2020, pp. 1241--1245.

\bibitem{DBLP:conf/cvpr/ZhukovACFLS19}
D.~Zhukov, J.~Alayrac, R.~G. Cinbis, D.~F. Fouhey, I.~Laptev, and J.~Sivic,
  ``Cross-task weakly supervised learning from instructional videos,'' in
  \emph{{CVPR}}.\hskip 1em plus 0.5em minus 0.4em\relax Computer Vision
  Foundation / {IEEE}, 2019, pp. 3537--3545.

\bibitem{DBLP:conf/cvpr/AlayracBASLL16}
J.~Alayrac, P.~Bojanowski, N.~Agrawal, J.~Sivic, I.~Laptev, and
  S.~Lacoste{-}Julien, ``Unsupervised learning from narrated instruction
  videos,'' in \emph{{CVPR}}.\hskip 1em plus 0.5em minus 0.4em\relax {IEEE}
  Computer Society, 2016, pp. 4575--4583.

\bibitem{DBLP:conf/cvpr/TangDRZZZL019}
Y.~Tang, D.~Ding, Y.~Rao, Y.~Zheng, D.~Zhang, L.~Zhao, J.~Lu, and J.~Zhou,
  ``{COIN:} {A} large-scale dataset for comprehensive instructional video
  analysis,'' in \emph{{CVPR}}.\hskip 1em plus 0.5em minus 0.4em\relax Computer
  Vision Foundation / {IEEE}, 2019, pp. 1207--1216.

\bibitem{DBLP:conf/iccv/MiechZATLS19}
A.~Miech, D.~Zhukov, J.~Alayrac, M.~Tapaswi, I.~Laptev, and J.~Sivic,
  ``Howto100m: Learning a text-video embedding by watching hundred million
  narrated video clips,'' in \emph{{ICCV}}.\hskip 1em plus 0.5em minus
  0.4em\relax {IEEE}, 2019, pp. 2630--2640.

\bibitem{DBLP:journals/corr/abs-2105-03404}
H.~Touvron, P.~Bojanowski, M.~Caron, M.~Cord, A.~El{-}Nouby, E.~Grave,
  A.~Joulin, G.~Synnaeve, J.~Verbeek, and H.~J{\'{e}}gou, ``Resmlp: Feedforward
  networks for image classification with data-efficient training,''
  \emph{CoRR}, vol. abs/2105.03404, 2021.

\bibitem{DBLP:conf/cvpr/EhsaniBRMF18}
K.~Ehsani, H.~Bagherinezhad, J.~Redmon, R.~Mottaghi, and A.~Farhadi, ``Who let
  the dogs out? modeling dog behavior from visual data,'' in
  \emph{{CVPR}}.\hskip 1em plus 0.5em minus 0.4em\relax Computer Vision
  Foundation / {IEEE} Computer Society, 2018, pp. 4051--4060.

\bibitem{DBLP:conf/iccvw/FarhaG19}
Y.~A. Farha and J.~Gall, ``Uncertainty-aware anticipation of activities,'' in
  \emph{{ICCV} Workshops}.\hskip 1em plus 0.5em minus 0.4em\relax {IEEE}, 2019,
  pp. 1197--1204.

\bibitem{DBLP:conf/cvpr/CarreiraZ17}
J.~Carreira and A.~Zisserman, ``Quo vadis, action recognition? {A} new model
  and the kinetics dataset,'' in \emph{{CVPR}}.\hskip 1em plus 0.5em minus
  0.4em\relax {IEEE} Computer Society, 2017, pp. 4724--4733.

\bibitem{DBLP:conf/cvpr/HeZRS16}
K.~He, X.~Zhang, S.~Ren, and J.~Sun, ``Deep residual learning for image
  recognition,'' in \emph{{CVPR}}.\hskip 1em plus 0.5em minus 0.4em\relax
  {IEEE} Computer Society, 2016, pp. 770--778.

\bibitem{Peebles2022DiT}
W.~Peebles and S.~Xie, ``Scalable diffusion models with transformers,''
  \emph{arXiv preprint arXiv:2212.09748}, 2022.

\bibitem{DBLP:conf/icassp/HersheyCEGJMPPS17}
S.~Hershey, S.~Chaudhuri, D.~P.~W. Ellis, J.~F. Gemmeke, A.~Jansen, R.~C.
  Moore, M.~Plakal, D.~Platt, R.~A. Saurous, B.~Seybold, M.~Slaney, R.~J.
  Weiss, and K.~W. Wilson, ``{CNN} architectures for large-scale audio
  classification,'' in \emph{{ICASSP}}.\hskip 1em plus 0.5em minus 0.4em\relax
  {IEEE}, 2017, pp. 131--135.

\bibitem{DBLP:journals/corr/KingmaB14}
D.~P. Kingma and J.~Ba, ``Adam: {A} method for stochastic optimization,'' in
  \emph{{ICLR} (Poster)}, 2015.

\bibitem{DBLP:journals/corr/abs-2205-14217}
X.~L. Li, J.~Thickstun, I.~Gulrajani, P.~Liang, and T.~B. Hashimoto,
  ``Diffusion-lm improves controllable text generation,'' \emph{CoRR}, vol.
  abs/2205.14217, 2022.

\bibitem{DBLP:conf/eccv/WuH18}
Y.~Wu and K.~He, ``Group normalization,'' in \emph{{ECCV} {(13)}}, ser. Lecture
  Notes in Computer Science, vol. 11217.\hskip 1em plus 0.5em minus 0.4em\relax
  Springer, 2018, pp. 3--19.

\bibitem{DBLP:journals/corr/abs-1908-08681}
D.~Misra, ``Mish: {A} self regularized non-monotonic neural activation
  function,'' \emph{CoRR}, vol. abs/1908.08681, 2019.

\bibitem{DBLP:conf/eccv/DvornikHPBMFJ22}
N.~Dvornik, I.~Hadji, H.~Pham, D.~Bhatt, B.~Mart{\'{\i}}nez, A.~Fazly, and
  A.~D. Jepson, ``Flow graph to video grounding for weakly-supervised
  multi-step localization,'' in \emph{{ECCV} {(35)}}, ser. Lecture Notes in
  Computer Science, vol. 13695.\hskip 1em plus 0.5em minus 0.4em\relax
  Springer, 2022, pp. 319--335.

\bibitem{DBLP:conf/nips/DvornikHDGJ21}
N.~Dvornik, I.~Hadji, K.~G. Derpanis, A.~Garg, and A.~D. Jepson, ``Drop-dtw:
  Aligning common signal between sequences while dropping outliers,'' in
  \emph{NeurIPS}, 2021, pp. 13\,782--13\,793.

\bibitem{DBLP:journals/tit/Viterbi67}
A.~J. Viterbi, ``Error bounds for convolutional codes and an asymptotically
  optimum decoding algorithm,'' \emph{{IEEE} Trans. Inf. Theory}, vol.~13,
  no.~2, pp. 260--269, 1967.

\bibitem{DBLP:conf/iclr/SongME21}
J.~Song, C.~Meng, and S.~Ermon, ``Denoising diffusion implicit models,'' in
  \emph{{ICLR}}.\hskip 1em plus 0.5em minus 0.4em\relax OpenReview.net, 2021.

\bibitem{stable_diff}
R.~Rombach, A.~Blattmann, D.~Lorenz, P.~Esser, and B.~Ommer, ``High-resolution
  image synthesis with latent diffusion models,'' in \emph{{CVPR}}.\hskip 1em
  plus 0.5em minus 0.4em\relax {IEEE}, 2022, pp. 10\,674--10\,685.

\bibitem{CLIP}
A.~Radford, J.~W. Kim, C.~Hallacy, A.~Ramesh, G.~Goh, S.~Agarwal, G.~Sastry,
  A.~Askell, P.~Mishkin, J.~Clark, G.~Krueger, and I.~Sutskever, ``Learning
  transferable visual models from natural language supervision,'' in
  \emph{{ICML}}, ser. Proceedings of Machine Learning Research, vol. 139.\hskip
  1em plus 0.5em minus 0.4em\relax {PMLR}, 2021, pp. 8748--8763.

% \bibitem{MoEs}
% R.~A. Jacobs, M.~I. Jordan, S.~J. Nowlan, and G.~E. Hinton, ``Adaptive mixtures
%   of local experts,'' \emph{Neural Comput.}, vol.~3, no.~1, pp. 79--87, 1991.
